Causal Matrix Completion

Matrix completion is the study of recovering an underlying matrix from a sparse subset of noisy observations. Traditionally, it is assumed that the entries of the matrix are "missing completely at random" (MCAR), i.e., each entry is revealed at random, independent of everything else, with uniform probability. This is likely unrealistic due to the presence of "latent confounders", i.e., unobserved factors that determine both the entries of the underlying matrix and the missingness pattern in the observed matrix. For example, in the context of movie recommender systems -- a canonical application for matrix completion -- a user who vehemently dislikes horror films is unlikely to ever watch horror films. In general, these confounders yield "missing not at random" (MNAR) data, which can severely impact any inference procedure that does not correct for this bias. We develop a formal causal model for matrix completion through the language of potential outcomes, and provide novel identification arguments for a variety of causal estimands of interest. We design a procedure, which we call "synthetic nearest neighbors" (SNN), to estimate these causal estimands. We prove finite-sample consistency and asymptotic normality of our estimator. Our analysis also leads to new theoretical results for the matrix completion literature. In particular, we establish entry-wise, i.e., max-norm, finite-sample consistency and asymptotic normality results for matrix completion with MNAR data. As a special case, this also provides entry-wise bounds for matrix completion with MCAR data. Across simulated and real data, we demonstrate the efficacy of our proposed estimator.

==> archived/applications.tex <==
\section{Other Applications} 

\begin{enumerate}
    \item Panel Data (e.g., SC)
    \begin{itemize}
        \item rows = units, columns = time 
        \item single intervention point (all units are under same intervention prior to this point) 
        \item $\theta_1^{(T)}$ = individual expected potential outcome at the single post-intervention period, $T$  
    \end{itemize}
    
    \item Causal Contextual Bandits, i.e., with Hidden Confounding
    \begin{itemize}
        \item rows = bandits, columns = context-action pairs
        \item $\theta_i^{(c, a)}$ = bandit-specific expected reward for every context-action pair
    \end{itemize}
    
    
    \item Deterministic RL 
    \begin{itemize}
        \item 
    \end{itemize}
\end{enumerate}

==> archived/assumptions.tex <==
\subsection{Observations}
%
\paragraph{Notation.}
For each unit $n$ and intervention $d$, define $\bm{1}_n^{(d)} \in \{0,1\}^T$, where 
$\bm{1}_{nt}^{(d)} = 1$ if $\Dc_{nt} = d$
where $\Dc_{nt} \in [D]$ is the ``intervention assignment'' for unit $n$ at time $t$.
% \begin{align}
% \end{align}

%
\paragraph{SUTVA.}
Define $Y_{nt}$ as the {\em observed outcome} of unit $n$ at time $t + 1$.
%
We assume,
% 
\begin{align}\label{eq:SUTVA}
Y_{nt} = 
%
\sum_{d}  \mathbbm{1}\{\Dc_{nt} = d\} 
%
\cdot Y^{(d)}_{nt},
\end{align}
%
In the RL setting, we note that $d$ is partially observed and partially selected, i.e., the state $x$ is observed while the action $a$ is selected.

\subsection{Latent Factor Model}
%
\paragraph{Time-varying LFM.}
%
Assume $Y^{(d)}_{nt}$ has the following factorization,
%
\begin{align}\label{eq:LFM}
Y^{(d)}_{nt} = \langle u^{(d)}_t, v_n \rangle + \varepsilon^{(d)}_{nt}, 
\end{align}
%
where $u^{(d)}_t \in \mathbb{R}^{r}$ is the latent factor associated with $d$ and $t$; 
%
$v_n \in \mathbb{R}^{r}$ is the latent factor associated with  unit $n$; 
%
$r$ implicitly captures the model complexity; 
% 
$\varepsilon^{(d)}_{nt}$ captures the `idiosyncratic shock' associated with the observation of unit $n$ at time $t$ under $d$. 
Without loss of generality, we will henceforth suppress dependencies on $d$ for the shocks $\varepsilon_{tn}$. 
%
Define,
%
\begin{align}\label{eq:conditioning_LF}
\LFc_t 
%
&\coloneqq 
%
\Big\{(v_n :  n \in [N]) \Big\} 
%
\cup \Big\{u^{(d)}_t:  d \in [D] \Big\} 
%
\end{align}
%
In words, $\LFc_t$ collects the unit and intervention latent factors till (and including) time step $t$.



%
\paragraph{Non Time-varying LFM.}
%
Assume $Y^{(d)}_{nt}$ has the following factorization,
%
\begin{align}\label{eq:RL_LFM}
Y^{(d)}_{nt} = \langle u^{(d)}, v_n \rangle + \varepsilon^{(d)}_{nt}, 
\end{align}
%
where $u^{(d)} \in \mathbb{R}^{r}$ is the latent factor associated with $d$ -- {\em crucially, there is no longer a dependence on $t$, as in RL, the expected potential outcome should only be a function of (state, action)}; 
%
$v_n \in \mathbb{R}^{r}$ is the latent factor associated with  unit $n$; 
%
$r$ implicitly captures the model complexity; 
% 
$\varepsilon^{(d)}_{nt}$ captures the `idiosyncratic shock' associated with the observation of unit $n$ at time $t$ under $d$. 
Without loss of generality, we will henceforth suppress dependencies on $d$ for the shocks $\varepsilon_{tn}$. 
%
Define,
%
\begin{align}\label{eq:RL_conditioning_LF}
\LFc 
%
&\coloneqq 
%
\Big\{(v_n :  n \in [N]) \Big\} 
%
\cup \Big\{(u^{(d)} :  d \in [D]  \Big\} 
%
\end{align}
%
In words, $\LFc$ collects the unit and intervention latent factors (again, there is no longer a dependence on $t$).
 

%
% We assume,
% %
% \begin{align}\label{eq:SUTVA}
% \tilde{Y}_{t, n} = 
% %
% \sum_{x_{t} \in \mathcal{X}} \ \sum_{a_{t} \in \mathcal{A}} \mathbbm{1}\Big\{X_{t, n} = x_{t}\Big\}\mathbbm{1}\Big\{\mathcal{D}_{t}(n) = a_{t}\Big\} 
% %
% Y^{(x, a)}_{t, n}
% \end{align}


==> archived/causal_matrix_estimation.tex <==
% \section{Target Causal Parameter}
% %
% \begin{itemize}
%     \item Potential outcomes framework + (LFM, SUTVA) 
%     \item Identification
%     \begin{itemize}
%         \item Target causal parameter
%         \item Assumptions on correlation between Sparsity pattern + Noise
%         \item Identification Argument
%     \end{itemize}
%     \item Meta-Algorithm -- identification argument informs which collection of rows, columns, slices are ``kosher''
% \end{itemize}

{\bf To-do's}
\begin{itemize}
    \item Re-organize + Abstract + condense
    \begin{itemize}
        \item Finish Reward + Time-varying LFM
        \item Causal matrix estimation 
    \end{itemize}
    \item Algorithm
\end{itemize}

\section{Potential outcomes framework}
%
Denote the target tensor as $\bM \in \Rb^{N \times D \times T}$ where $M_{ndt} = Y^{(d)}_{nt}$.
%
Here, $Y^{(d)}_{nt}$ denotes the potential outcome of unit $n$ under intervention $d$ at time $t$.
%

{\bf Example 1: Reinforcement Learning.}
Let $d = (x, a) \in [\Xc] \times [\Ac]$, where $\Xc, \Ac$ refers to the collection of states and actions, respectively;
%
$T$ refers to the length of the episode.
% 
Let $X_{nt} \in \mathcal{X}$ denote the random variable (r.v.) that represents the state of unit $n$ at time $t$.
%
Let $A_{nt} \in \mathcal{A}$ denote the r.v. that represents the action unit $n$ receives at time $t$.
%
Let $R_{nt} \in \Rb$ denote the r.v. that represents the reward unit $n$ receives at time $t$. 

{\em Simulator. } 
Here, $Y^{(x, a)}_{nt}$ is the conditional expected transitional state under a ``do'' operation of unit $n$ at time step $t+1$, i.e.,
$$
Y^{(x, a)}_{nt} \coloneqq \Ex[X_{n,t+1} \ | \ X_{nt} = x, ~\text{do}(A_{nt} = a)].
$$

{\em Reward. }
Here, $Y^{(x, a)}_{nt}$ is the conditional expected reward/rating/revenue-generated under a ``do'' operation of unit $n$ at time step $t$, i.e.,
$$
Y^{(x,a)}_{nt} \coloneqq \Ex[R_{nt} \ |  \ X_{nt} = x, ~\text{do}(A_{nt} = a)].
$$


% {\bf Example 1: Reinforcement Learning.}
% %
% Here $d = (x, a) \in [\Xc] \times [\Ac]$, where $\Xc, \Ac$ refers to the collection of states and actions, respectively;
% %
% $T$ refers to the length of the episode.
% %
% As an example,
% %
% $Y^{(x, a)}_{nt}$ is the conditional expected transitional state under a ``do'' operation of unit $n$ at time step $t+1$, i.e.,
% $$
% Y^{(x, a)}_{nt} \coloneqq \Ex[X_{n,t+1} \ | \ X_{nt} = x, ~\text{do}(A_{nt} = a)]
% $$


% {\bf Example 2: Recommendation Systems. } 
% %
% As a concrete example, $d$ represents products, movies, etc. 
% %
% $T$ refers to the the number of time steps the platform gets to make recommendations to its users.
% %
% As an example,
% %
% $Y^{(d)}_{nt}$ is the conditional expected reward/rating/revenue-generated under a ``do'' operation of unit $n$ at time step $t$, i.e.,
% $$
% Y^{(d)}_{nt} \coloneqq \Ex[R_{nt} \ |  \ X_{nt} = x, ~\text{do}(A_{nt} = a)]
% $$




==> archived/model.tex <==

\section{Connecting SI and mSSA with Linear Control}
%
\subsection{Innovation Model}
%
Let there be $N \in \Nb$ units, $T \in \Nb$ time steps, and $I \in \Nb$ interventions. 

Let $\Delta \in \Rb^{N \times T \times I}$ be a 3-dimensional tensor, where $\Delta_{(n, i)}(t)$ denotes the innovation for unit $n \in [N]$, $t \in [T]$, $i \in [I]$.

\subsection{Observation Model}
%
\subsubsection{Noiseless Observations}
%
For a particular unit $n$, if it receives a sequence of interventions $\{i_{(n ,1)}, \dots, i_{(n ,t)} \}$ where each $i_{(\cdot, \cdot)} \in [I]$, we observe
%
\begin{align}\label{eq:dynamics}
%
M_{(n)}(t) = M_{(n)}(t - 1) + f\left(\Delta_{(n,  i_{(n ,1)})}(t), \ \dots, \ \Delta_{(n,  i_{(n ,t)})}(t)\right)
%
\end{align}
%

\subsubsection{Noisy Observations}
%
We observe 
\[
Y_{(n)}(t) = M_{(n)}(t) + \varepsilon_{(n)}(t)
\]


\subsection{Assumptions}\label{sec:assumptions}
%
\begin{enumerate}
\item $\Delta$ is a low-rank tensor, i.e., 
%
\begin{align}\label{eq:low_rank_tensor_assumption}
\Delta_{(n, i)}(t) = \sum^{R}_{r=1} \theta_{(n, r)}  \omega_{(i, r)} \rho_{(r)}(t) 
\end{align}
%
\item $\rho_{(r)}(t)$ follows a Linear Recurrent Formula (LRF), i.e.,
%
\begin{align}\label{eq:LRF_assumption}
\rho_{(r)}(t) = \sum^{G}_{g=1} \beta_{(r, g)} \rho_{(r)}(t - g) 
\end{align}
%
\item  $f$ is a linear response model, i.e.,
%
\begin{align}\label{eq:linear_response_assumption}
%
 f\left(\Delta_{(n,  i_{(n ,1)})}(1), \ \dots, \ \Delta_{(n,  i_{(n ,t)})}(t)\right) 
%
= \sum^{t}_{k=1} \alpha(i_{(n, k)}, t - k) \cdot \Delta_{(n, i_{(n, k)})}(t)
%
\end{align}
% 
where $  \alpha(i_{(n, k)}, t - k)$ is a function of the intervention $i_{(n, k)}$ and the time difference $t - k$.
%
\end{enumerate}

\subsection{Spatio-Temporal Tensor Factor Model as a Linear Dynamical System}
%
%\begin{prop}
%%
%Let Assumptions (1) and (2) from Section \ref{sec:assumptions} hold.
%%
%For all $n \in [N]$, $i \in [I]$,
%%
%\begin{align}
%%
%\Delta_{(n, i)}(t) = \sum^{G}_{g = 1} \beta_g \Delta_{(n, i)}(t - g) 
%%
%\end{align}
%%
%\end{prop}
%%
%\begin{proof}
%%
%\begin{align}
%%
%\Delta_{(n, i)}(t) 
%%
%&= \sum^{R}_{r=1} \theta_{(n, r)}  \omega_{(i, r)} \rho_{(r)}(t) 
%%
%\\ &= \sum^{R}_{r=1} \theta_{(n, r)}  \omega_{(i, r)}  \left(\sum^{G}_{g=1} \beta_g \rho_{(r)}(t - g)\right)
%%
%\\ &= \sum^{G}_{g=1} \beta_g  \sum^{R}_{r=1} \theta_{(n, r)}  \omega_{(i, r)}  \rho_{(r)}(t - g)
%%
%\\ &= \sum^{G}_{g=1} \beta_g  \Delta_{(n, i)}(t - g) 
%%
%\end{align}
%%
%\end{proof}

\subsubsection{Writing $\Delta_{n, i}$ as a dynamical system.}
%
%A linear dynamical system is one which can be written as 
%%
%\begin{align}
%%
%X(t + 1) &= \bA X(t) + \bB u(t + 1)
%%
%\\ Y(t + 1) &= \bC X(t + 1) + \bD w(t + 1)
%%
%\end{align}
%

For $r \in [R]$, define $\bA_{(r)} \in \Rb^{G \times G}$ and $X_{(r) (\cdot)} \in \Rb^{G}$ as,
%
\begin{align}
%
\bA_{(r)} = 
%
\begin{bmatrix} 
%
\beta_{(r, 1)} &  \beta_{(r, 1)} & \dots & \beta_{(r, G)}  \\
%
1 &  0 & \dots  \\
%
0 & 1 &  \dots \\
%
\vdots & \ddots & \\
%
0 &     \dots  & 1 & 0
%
\end{bmatrix}
%
, \quad X_{(r)}(t) = 
%
\begin{bmatrix} 
%
\rho_{(r)}(t) \\
%
\vdots \\
%
\rho_{(r)}(t - G + 1) 
%
\end{bmatrix}
%
\end{align}
%
Define $\bA \in \Rb^{RG \times RG}$ and $X(\cdot) \in  \Rb^{RG}$
%
\begin{align}
%
\bA =
%
\begin{bmatrix}
    \, \bA_{(1)} & 0 & 0\,  \\
    \, 0 & \bA_{(2)} & 0 & \hdots \, \\
    \,0 & 0 & \bA_{(3)}\, \\
    \, & \vdots&& \ddots \, \\
    \, & &&&  \bA_{(R)}\, \\
  \end{bmatrix}
  %
  , \quad X(t) = 
%
\begin{bmatrix} 
%
X_{(1)}(t) \\
%
\vdots \\
%
X_{(R)}(t) 
%
\end{bmatrix}
\end{align}
%
\begin{proposition}\label{prop:LRF_LTI}
%
Let Assumption \eqref{eq:LRF_assumption} from Section \ref{sec:assumptions} hold.
%
Then,
%
\begin{align}
X(t+1) = \bA X(t)
\end{align}
\end{proposition}
%
\begin{proof}
%
Immediate.
%
\end{proof}

Write $\bB \in \Rb^{NI \times RG}$ as,
%
\[
\bB_{(n, i), \cdot} =  \left[\left(\theta_{(n, 1)} \omega_{(i, 1)}, \ 0, \ \dots, \ 0\right), \ \dots,  \left(\theta_{(n, R)} \omega_{(i, R)}, \ 0, \ \dots, \ 0\right) \right]
\]
%
Write 
%
$Y(\cdot) \in \Rb^{NI}$ as,
%
\[
Y(t) =
\begin{bmatrix}
%
\Delta_{1, 1}(t) \\
%
\Delta_{1, 2}(t) \\
%
\vdots \\
%
\Delta_{N, I - 1}(t) \\
%
\Delta_{N, I}(t)
%
\end{bmatrix}
\]
%
\begin{proposition}
%
Let Assumption \eqref{eq:low_rank_tensor_assumption} from Section \ref{sec:assumptions} hold.
%
Then,
%
\begin{align}
%
Y(t) = \bB X(t)
%
\end{align}
%
\end{proposition}
%
\begin{proof}
%
Immediate.
%
\end{proof}

Define $\Delta^{\text{obs}}(\cdot) \in \Rb^{N}$ as,
%
\[
\Delta^{\text{obs}}(t) =
%
\begin{bmatrix}
%
\Delta_{(1, i_{(1, t)})}(t) \\
%
\vdots \\
%
\Delta_{(N, i_{(N, t)})}(t)
%
\end{bmatrix}
\]

Define $C_{(n)}(\cdot) \in \Rb^{1 \times I}$ as,
%
\[
[C_{(n)}(t)]_{j} = 
\begin{cases}
1, \quad \text{if} \ j = i_{(n, t)} \\
0, \quad \text{otherwise}
\end{cases}
\]
%
Define $\bC(\cdot) \in \Rb^{N \times NI}$ as,
%
\[
\bC(t) = 
%
\begin{bmatrix}
\, C_{(1)}(t) & 0 & 0\,  \\
    \, 0 & C_{(2)}(t) & 0 & \hdots \, \\
    \,0 & 0 & C_{(3)}(t) \, \\
    \, & \vdots&& \ddots \, \\
    \, & &&&  C_{(N)}(t) \, \\
\end{bmatrix}
\]

\begin{proposition}\label{prop:delta_obs_LTI}
%
Let Assumptions \eqref{eq:low_rank_tensor_assumption} and \eqref{eq:LRF_assumption} from Section \ref{sec:assumptions} hold.
%
Then,
%
\begin{align}
%
\Delta^{\text{obs}}(t) = \bC(t) Y(t) = \bC(t)  \bB X(t) = \bC(t) \bB \bA X(t - 1)
%
\end{align}
%
\end{proposition}
%
\begin{proof}
Immediate.
\end{proof}

%%
%\begin{remark}
%%
%The potential outcomes framework and control have different notions of ``intervention''.
%%
%Potential outcomes framework posits that there are many latent dynamical trajectories that are evolving and an intervention causes us to ``jump'' to a particular latent trajectory.
%%
%This is captured implicitly through the matrix $\bC(\cdot)$.
%
%% 
%In control, it is the $u(t)$ that is driving the system.
%%
%So we see that when trying to connect (at least naively), the potential outcomes lens to the control lens, it leads to $u(t) = 0$, which feels a little dissatisfying.
%\end{remark}

\subsection{Writing $M(t)$ as a dynamical system.}
%
Define $M(t) \in \Rb^{N}$ 
\[
M(t) =
\begin{bmatrix}
%
M_{(1)}(t) \\
%
M_{(2)}(t)  \\
%
\vdots \\
%
M_{(N)}(t)
%
\end{bmatrix}
\]
%
Define $\widetilde{X}(t) \in \Rb^{N + RG}$ as
\[
\widetilde{X}(t) =
%
\left(
    \begin{array}{c}
      M(t)\\
      \hline
      X(t)
    \end{array}
    \right)
\]

\begin{proposition}
Assume \eqref{eq:dynamics} holds.
%
Further assume,
\[
f\left(\Delta_{(n,  i_{(n ,1)})}(t), \ \dots, \ \Delta_{(n,  i_{(n ,t)})}(t)\right) = \Delta_{(n,  i_{(n ,t)})}(t).
\]
%
Then we can express $\widetilde{X}(t)$ as 
\[
\widetilde{X}(t) =
%
\left(
    \begin{array}{c}
      M(t)\\
      \hline
      X(t)
    \end{array}
\right)
%
= \left(
    \begin{array}{c|c}
      \bI & \bC(t)  \bB \bA \\
      \hline
      \boldsymbol{0} & \bA
    \end{array}
    \right) \left(
    \begin{array}{c}
      M(t -1)\\
      \hline
      X(t -1)
    \end{array}
\right)
\]
\end{proposition}

\begin{proof}
Holds immediately from \eqref{eq:dynamics}, the assumptions of the proposition, and the identities established in Propositions \ref{prop:LRF_LTI} and \ref{prop:delta_obs_LTI}.
\end{proof}

\begin{remark}
%
We note that $\bA, \bB$ are latent matrices define by the LRF and Tensor Factor model, respectively.
%
The control applied at time $t$ is $\bC(t)$ which is a matrix of $\{0, 1\}$, where a non-zero entry serves as an indicator that control was applied to a particular unit at time $t$, i.e. it encodes $i_{(n, t)}$ for $n \in [N]$.
%
Thus $C(t)$ serves as `proxy' $u(t)$ as written in LTI language, where $u(t)$ in this formalism is not allowed to be an abritrary real-valued number as is commonly assumed.
\end{remark}

\begin{remark}
Replacing $\bI$ with a low-rank matrix for top left-hand corner might be a natural way to incorporate ``network effect'' in causal models.
\end{remark}
%\begin{remark}
%Define $\Theta_{n} \in \Rb^{I \times R}$, where $[\Theta_{n}]_{i, \cdot} = [\theta_{(n, 1)}, \ \dots,  \ \theta_{(n, R)}]$.
%%
%Define $\Omega \in \Rb^{I \times R}$ where $\Omega_{i, r} = \omega_{(i, r)}$.
%%
%Then,
%%
%\[
%\bB = 
%%
%\begin{bmatrix}
% \, \Omega & 0 & 0\,  \\
%    \, 0 & \Omega & 0 & \hdots \, \\
%    \,0 & 0 & \Omega\, \\
%    \, & \vdots&& \ddots \, \\
%    \, & &&&  \Omega\, \\
%\end{bmatrix} 
%\circ
%\begin{bmatrix}
% \, \Theta_{1} & 0 & 0\,  \\
%    \, 0 & \Theta_{2} & 0 & \hdots \, \\
%    \,0 & 0 & \Theta_{3}\, \\
%    \, & \vdots&& \ddots \, \\
%    \, & &&&  \Theta_{N}\, \\
%\end{bmatrix} 
%\]
%\end{remark}
%
%{
%\begin{remark}
%%
%Consider the special case where 
%%
%\[
%%
% f\left(\Delta_{(n,  i_{(n ,1)})}(1), \ \dots, \ \Delta_{(n,  i_{(n ,t)})}(t)\right) 
% %
%= \Delta_{(n, i_{(n, t)})}(t)
%%
%\]
%%
%Then one can verify through recursion that,
%%
%\[
%M_n(t) = 
%%
%[1, \dots, 0] \left[ X_{(n, i_{(n, 1)})}(1) +  \bA X_{(n, i_{(n, 2)})}(1)  + \dots + \bA^{t-1} X_{(n, i_{(n, t)})}(1)\right]
%%
%\]
%\end{remark}
%}

%
\subsection{Goal}
%
Given observations $Y_{(n)}(t)$, for $n \in [N]$ and $t \in [T_0]$   

\subsubsection{Estimate $f$ and Forecast $\Delta$}
%
\begin{enumerate}
%
\item Assume $f$ is known, forecast $\Delta_{(n, i)}(t)$ for $t \in \{T_0, T\}$, $n \in [N]$, $i \in [I]$
%
\item Assume $f$ is Linear, Estimate $f$ and forecast $\Delta_{(n, i)}(t)$ for $t \in \{T_0, T\}$, $n \in [N]$, $i \in [I]$
%
\end{enumerate}
%

\subsection{Control Policy}
%
\begin{enumerate}
%
\item Given a reward function 
\[
R: (f, \Delta) \to \Rb,
\]
estimate optimal sequence of interventions $\{i^{n}_{t}\}_{n \in [N], t \in  \{T_0, T\}}$.
%
\end{enumerate}

\section{Assume $f$ is known, forecast $\Delta_{n, t, i}$: SI + mSSA}




==> archived/selection_latent.tex <==
\section{Selection on Latent Factors -- Causal DAG Viewpoint}\label{sec:causal_dag_LFM}


\subsection{Causal DAG Identification with Selection on Latent Factors}
%
Recall from \eqref{eq:conditioning} that
\[
\Ec_t \coloneqq  \Big\{(u^{(x_{t'}, a_{t'})}: \ x_{t'} \in \mathcal{X}, \ a_{t'} \in \mathcal{A}, \ t' \le t), \ (v_n\ n \in [N]) \Big\}.
\]
%
Then,
{\small
%
\begin{align}
%
&\mathbb{P}^{\text{do}(A_{t, n} = a_{t, n})}\Big(X_{t+1, n} = x_{t+1, n} | X_{t, n} = x_{t, n}, \ \Ec_t \Big)
%
\\ &\stackrel{(a)} = \sum_{\tilde{a}_{t, n}} \ \sum_{\tilde{\epsilon}_{t, n}} \mathbb{P}^{\text{do}(A_{t, n} = a_{t, n})}\Big(X_{t+1} = x_{t+1}, \ \epsilon_{t, n} =\tilde{\epsilon}_{t, n} , \ A_{t, n} = \tilde{a}_{t, n} | X_{t, n} = x_{t, n},  \ \Ec_t \Big),
%
\\ &\stackrel{(b)} = \sum_{\tilde{a}_{t, n}} \ \sum_{\tilde{\epsilon}_{t, n}}  \bigg\{ \mathbb{P}^{\text{do}(A_{t, n} = a_{t, n})}\Big(X_{t+1, n} = x_{t+1, n} | X_{t, n} = x_{t, n}, \  \epsilon_{t, n} =\tilde{\epsilon}_{t, n}, \ A_{t, n} = \tilde{a}_{t, n},  \ \Ec_t\Big) 
\\ &  \qquad \qquad \qquad\mathbb{P}^{\text{do}(A_{t, n} = a_{t, n})}\Big( \epsilon_{t, n} =\tilde{\epsilon}_{t, n}, \ A_{t, n} = \tilde{a}_{t, n} | X_{t, n} = x_{t, n},  \ \Ec_t\Big) \bigg\},
%
\\ &\stackrel{(c)} = \sum_{\tilde{a}_{t, n}} \ \sum_{\tilde{\epsilon}_{t, n}} \bigg\{ \mathbb{P}^{\text{do}(A_{t, n} = a_{t, n})}\Big(X_{t+1, n} = x_{t+1, n} | X_{t, n} = x_{t, n}, \ \epsilon_{t, n} =\tilde{\epsilon}_{t, n}, \ A_{t} = \tilde{a}_{t, n},  \ \Ec_t\Big)  
\\ & \qquad \qquad \qquad \quad \mathbb{P}^{\text{do}(A_{t, n} = a_{t, n})}\Big(A_{t} = \tilde{a}_{t, n} | \epsilon_{t, n} =\tilde{\epsilon}_{t, n}, \ X_{t, n} = x_{t, n},  \ \Ec_t\Big) 
\\ & \qquad \qquad \qquad \quad \mathbb{P}\Big(\epsilon_{t, n} =\tilde{\epsilon}_{t, n} | X_{t, n} = x_{t, n},  \ \Ec_t\Big) \bigg\},
%
\\ &\stackrel{(d)} = \sum_{\tilde{\epsilon}_{t, n}} \bigg\{\mathbb{P}\Big(X_{t+1, n} = x_{t+1, n} | X_{t, n} = x_{t, n}, \ \epsilon_{t, n} =\tilde{\epsilon}_{t, n}, \ A_{t, n} = a_{t, n},  \ \Ec_t\Big) 
\\ & \qquad \qquad \qquad \quad\mathbb{P}\Big(\epsilon_{t, n} =\tilde{\epsilon}_{t, n} | X_{t, n} = x_{t, n},  \ \Ec_t\Big) \bigg\},
%
\\ &\stackrel{(e)} = \sum_{\tilde{\epsilon}_{t, n}} \bigg\{\mathbb{P}\Big(X_{t+1, n} = x_{t+1, n} | X_{t, n} = x_{t, n}, \ \epsilon_{t, n} =\tilde{\epsilon}_{t, n}, \ A_{t, n} = a_{t, n},  \ \Ec_t\Big) 
\\ & \qquad \qquad \qquad \quad\mathbb{P}\Big(\epsilon_{t, n} =\tilde{\epsilon}_{t, n} | X_{t, n} = x_{t, n}, \ A_{t, n} = a_{t, n}, \ \Ec_t\Big) \bigg\},
%
\\ &\stackrel{(f)} = \{\mathbb{P}\Big(X_{t+1, n} = x_{t+1, n} | X_{t, n} = x_{t, n},  \ A_{t, n} = a_{t, n},  \ \Ec_t\Big) 
%%\\ &{\color{red} \qquad \quad \quad  \mathbb{P}\Big(A_{t, n} = a_{t, n} | U_{t} = \tilde{u}_{t}, \ X_{t, n} = x_{t, n}\Big)}
%\mathbb{P}\Big(\epsilon_{t, n} =\tilde{\epsilon}_{t, n} | X_{t, n} = x_{t, n}\Big) \bigg\} \label{eq:final_select_observabales},
\end{align}
 }
where (a) is by definition of marginalization; (b) and (c) are by definition of conditional probability; (d) is by ``do''-calculus; (e) is by the conditional independences induced by the DAG; (f) is by definition of marginalization. \\

\subsection{Algorithm Overview}
%
{\bf Goal}: For unit $n$, produce the counterfactual state $X_{n, t+1}$ given that at time $t$, it is at state $X_{n, t} = x_{t}$ and we $\text{do}(A_{n, t} = a_{t})$.

%
{\bf Observations}: A single $T$ time step trajectory, $X_{n, 1} \to A_{n, 1} \to X_{n, 2} \dots X_{n, T}$ for each unit $n$.

%
{\bf Proposed Algorithm}: Given the identification argument in Section \ref{sec:identification_LFM_potential_outcomes}, below is a proposal
%
\begin{itemize}

	\item Donor Group Selection
	\begin{itemize}
		%\item Collect all other units $j \in [N]$ such that there exists $t_j \in [T]$, where $X_{j, t_j} = x_{t}$ and action $A_{j, t_j} = a_{t}$. Denote this group as $\Ic^{(x_t, a_t)}$.
		
		\item Define  
		$$
		\Ic^{(x_t, a_t)} = \{j \in [N]: \text{unit } j \text{ experienced } (x_t, a_t) \text{ at some } t \in [T]\}.
		$$  
		
		\item For each subset of units $\mathcal{G} \subset  \Ic^{(x_t, a_t)}$, compute maximum number of overlapping (state, action) pairs with target unit $n$, i.e., 
		\begin{align}
		X_{\mathcal{G}} &= \{ x  :  \exists a \text{ s.t. } \forall j \in \mathcal{G} ~\exists~ t_n, t_j \text{ s.t. } X_{n, t_n} = X_{j, t_j} = x \text{ and } A_{n, t_n} = A_{j, t_j} = a \},
		\end{align}  
		with $T_{\mathcal{G}} = | X_{\mathcal{G}} |$. 
		
		
		%\item For each subset of units $\mathcal{G} \subset  \Ic^{(x_t, a_t)}$, compute the maximum size of overlap with unit $n$, i.e.,  for each $j \in \mathcal{G}$ there exist $t'_n$ and $t'_j$ such that $X_{n, t'_n} = X_{j, t'_j} $ {\em and} $A_{n, t'_n} = A_{j, t'_j} $. Denote the number of overlapping (state, action) pairs as $N_{\mathcal{G}}$.
		
		\item Find $\mathcal{G}^{*}$ such that $N_{\mathcal{G}}$ and $|\mathcal{G}|$ are ``sufficiently'' large. This is the donor group. That is, 
		$$\mathcal{G}^{*} = \argmax_{\mathcal{G} \subset  \Ic^{(x_t, a_t)}} \min(T_{\mathcal{G}}, |\mathcal{G}|).
		$$
		
		%\item $\mathcal{G}^{*}$ is the donor group the maximizes the minimum of the number of donors, $|\mathcal{G}|$, and the size of the overlap, $N_{\mathcal{G}}$.
	\end{itemize}
	
	\item SI: 
	\begin{itemize}
% 	    \item Let $y_n = [X_{n, t_1}, \dots, X_{n, t_{T_{\mathcal{G}}}}]$ denote  
		
% 		\item Model learning: 
		
% 		\item Counterfactual Prediction: 
		
		\item Given donor group $\mathcal{G}^{*}$, build SI model using the states in the overlap. 
		\item Apply model to estimate $X_{n, t+1}$
		\item {\color{blue} Notation not finalized yet}
	\end{itemize}
\end{itemize}

\subsection{Questions}
\begin{itemize}
    \item Target causal parameter:
    \begin{itemize}
        \item Real-valued vs. Distribution?
        \item Defined only for time $t$ or for an arbitrary state-action pair $(x, a)$?
    \end{itemize}
    \item State observations: Discrete vs. Continuous vs. Distributions?
    \item Should we include $K$, the number of time a state has been revisited, as a parameter? 
\end{itemize}

\newpage
\subsection{Causal DAG for other Potential Outcomes}
%
What happens if we let $Y^{(x, a)}_{t, n}$ equal the following quantities?
%
\begin{align}
%
\Ex[Y^{(x, a)}_{t, n}] &\coloneqq \text{Q-Learning}_n(x_t, a_t)
%
\\ \Ex[Y^{(x, a)}_{t, n}] &\coloneqq \text{Reward}_n(x_t, a_t)
\end{align}
%
Is it true that $\text{Q-Learning}_n(x_t, a_t)$ and $\text{Reward}_n(x_t, a_t)$ do not affect $X_n(t + 1)$.
%
This would lead to the following Causal DAG. 
%
Can we weaken the assumptions made/change the algorithm for this case?



\subsubsection{RL-Learning Specific Causal Parameter}
%
\paragraph{``Algorithm Free'' Causal Parameter}
%
In the previous section, recall the target parameter was $Y^{(x, a)}_{t, n}$.
%
Hence, $\Ex[Y^{(x, a)}_{t, n}]$ is dependent on $x$, $a$, and $n$.
%
An advantage of defining our potential outcome in this fashion is that it is ``algorithm--free''.
%
A disadvantage is that it requires defining a potential outcome for each $x$, $a$ and unit $n$.
%
This reduces the number of feasible donors.
%
In particular, recalling that $R$ is the model complexity, for \eqref{eq:linear_span} to hold we require 
\[
|\mathcal{I}^{(x_t, a_t)}| \ \gg \ R.
\]


%
\paragraph{``RL-Algorithm Specific'' Causal Parameter}
%
Another possible strategy is to define a ``RL-algorithm specific'' causal parameter.
%
Say for instance we know a priori our downstream RL learning policy will be learnt via $Q$-learning.
%
We then define 
%
\[
[Y_{\text{Q-Learning}}^{(x_t, a_t)}]_{t, n}, \ \text{for} \ x_t \in \mathcal{X}, \ a_t \in \mathcal{A}, \ n \in [N].
\]
%
Such a formulation might move some of the complexity to the specifics of the RL algorithm used.
%
Say a RL algorithm never explores a particular action or state, then we might require less estimation accuracy for that potential outcome.
%
%In the particular case of Q-learning, which only requires learning the discounted reward for any state and action pair, $x \in \mathcal{X}, a \in \mathcal{A}$, we can index our potential outcome only by $x \in \mathcal{X}, \ a \in \mathcal{A}, \ n \in [N]$. 
%
Observe that $[Y_{\text{Q-Learning}}^{(x_t, a_t)}]_{t, n}$ is  in line with the target parameter in \textit{``Sample Efficient Reinforcement Learning via Low-Rank Matrix Estimation''} by Shah, Song, Xu, and Yang.
%
There are two meaningful generalizations we should tackle: 
\begin{enumerate}
	%
	\item We do not get to arbitrarily sample from this $\mathbb{R}^{|\mathcal{X}| \times |\mathcal{A}| \times N}$ 3-dimensional tensor -- the pattern of missingness and/or the noise in the observations may be {\em confounded} with the potential outcome, i.e.,  $[Y_{\text{Q-Learning}}^{(x_t, a_t)}]_{t, n}$ is correlated with $\epsilon_{xan}$. 
	%
	\begin{enumerate}
		%
		\item Here $\epsilon_{xan}$ is analogous to \eqref{eq:LFM}, i.e., the residual after we factorize $[Y_{\text{Q-Learning}}^{(x_t, a_t)}]_{t, n}$. In particular,
		\[
		 [Y_{\text{Q-Learning}}^{(x_t, a_t)}]_{t, n} = \sum^{R}_{r = 1} \theta_{xr} \rho_{ar} \omega_{nr} + \epsilon_{xan}
		\]
		%
	\end{enumerate}
	%
	\item We now want to learn {\em across units}, formalized by the additional indexing by $n \in [N]$. This will allow us to: (i) circumvent selection on unobservables; (ii) increase sample complexity.
	%
\end{enumerate}


==> archived/selection_observables.tex <==
\section{Sequential Selection on Observables}

\subsection{Selection on Observables -- Causal DAG Viewpoint} 
\begin{tikzpicture}
	% nodes %
	\node[text centered] (x1) {$X_{t}$};
	\node[right = 1.5 of x1, text centered] (u1) {$U_{t}$};
	\node[right=1.5 of u1, text centered] (a1) {$A_{t}$};
	\node[right=1.5 of a1, text centered] (x2) {$X_{t+1}$};

	% edges %
	\path (x1) edge (u1);
	\path (u1) edge (a1);
	\path (a1) edge (x2);
	\path (x1) edge[bend left=20] (a1);
	\path (x1) edge[bend left=20] (x2);
	\path (u1)  edge[bend right=20] (x2); 
\end{tikzpicture}

where $X_{t} \in \mathcal{X}$, $U_{t} \in \mathcal{U}$, and $A_{t} \in \mathcal{A}$, for all $t \in [T]$ and $n \in [N]$.

%
\paragraph{Interpretation and Example.}
%
\begin{itemize}
	%
	\item $X_{t}$ is the state at time $t$
	\begin{itemize}
		\item e.g. $X_{t}$ is the blood pressure of an individual on the start of day $t$
	\end{itemize} 
	%
	\item $U_{t}$ is a confounder at time $t$, which is affected by state $X_{t}$ 
	\begin{itemize}
		\item  e.g. $U_{t}$ is whether an individual exercises on day $t$ which is affected by his or her blood pressure at the start of day $t$
	\end{itemize} 
	%
	\item $A_{t} \in \mathcal{A}$ is the action at time $t$, which is affected by state $X_{t}$ and confounder  $U_{t}$
	\begin{itemize}
		\item e.g. $A_{t}$ is whether an individual diets on day $t$ which is affected by blood pressure and whether or not one exercises on day $t$
	\end{itemize} 
	%
	\item $X_{t+1}$ the state at time $t + 1$  
	\begin{itemize}
		\item e.g. $X_{t+1}$ is blood pressure on the start of day $t+1$ which is affected by blood pressure. whether one exercised, and whether on dieted on day $t$
	\end{itemize}
	%
\end{itemize}

\subsection{Causal DAG Identification with Selection on Observables}
{\small
%
\begin{align}
%
&\mathbb{P}^{\text{do}(A_{t} = a_{t})}\Big(X_{t+1} = x_{t+1} | X_{t} = x_{t}\Big)
%
\\ &\stackrel{(a)} = \sum_{\tilde{a}_{t} \in \mathcal{A}} \ \sum_{\tilde{u}_{t} \in \mathcal{U}} \mathbb{P}^{\text{do}(A_{t} = a_{t})}\Big(X_{t+1} = x_{t+1}, \ U_{t} = \tilde{u}_{t}, \ A_{t} = \tilde{a}_{t} | X_{t} = x_{t}\Big),
%
\\ &\stackrel{(b)} = \sum_{\tilde{a}_{t} \in \mathcal{A}} \ \sum_{\tilde{u}_{t} \in \mathcal{U}}  \bigg\{ \mathbb{P}^{\text{do}(A_{t} = a_{t})}\Big(X_{t+1} = x_{t+1} | X_{t} = x_{t}, \ U_{t} = \tilde{u}_{t}, \ A_{t} = \tilde{a}_{t}\Big) 
\\ &  \qquad \qquad \qquad\mathbb{P}^{\text{do}(A_{t} = a_{t})}\Big(U_{t} = \tilde{u}_{t}, \ A_{t} = \tilde{a}_{t} | X_{t} = x_{t}\Big) \bigg\},
%
\\ &\stackrel{(c)} = \sum_{\tilde{a}_{t} \in \mathcal{A}} \ \sum_{\tilde{u}_{t} \in \mathcal{U}} \bigg\{ \mathbb{P}^{\text{do}(A_{t} = a_{t})}\Big(X_{t+1} = x_{t+1} | X_{t} = x_{t}, \ U_{t} = \tilde{u}_{t}, \ A_{t} = \tilde{a}_{t}\Big)  
\\ & \qquad \qquad \qquad \quad \mathbb{P}^{\text{do}(A_{t} = a_{t})}\Big(A_{t} = \tilde{a}_{t} | U_{t} = \tilde{u}_{t}, \ X_{t} = x_{t}\Big) 
\\ & \qquad \qquad \qquad \quad \mathbb{P}^{\text{do}(A_{t} = a_{t})}\Big(U_{t} = \tilde{u}_{t} | X_{t} = x_{t}\Big) \bigg\},
%
\\ &\stackrel{(d)} = \sum_{\tilde{u}_{t}} \bigg\{\mathbb{P}\Big(X_{t+1} = x_{t+1} | X_{t} = x_{t}, \ U_{t} = \tilde{u}_{t}, \ A_{t} = a_{t}\Big) 
%\\ &{\color{red} \qquad \quad \quad  \mathbb{P}\Big(A_{t} = a_{t} | U_{t} = \tilde{u}_{t}, \ X_{t} = x_{t}\Big)}
\mathbb{P}\Big(U_{t} = \tilde{u}_{t} | X_{t} = x_{t}\Big) \bigg\} \label{eq:final_select_observabales},
\end{align}
}
where (a) is by definition of marginalization; (b) and (c) are by definition of conditional probability; (d) is by ``do''-calculus \\

\begin{remark}
If we get to observe the confounder $U_t$, then we can appropriately re-weigh the naive factorization 
\[
\mathbb{P}(X_{t+1} = x_{t+1} | X_{t} = x_{t}, \ A_{t} = a_{t})
\]
by \eqref{eq:final_select_observabales}. This is essentially sequential selection on observables.
\end{remark}


==> archived/tensor_factor_model.tex <==
\section{Latent Factor Model Viewpoint}
%
Consider the following data representation:
$\bM \in \Rb^{N \times (|\Sc||\Ac|)}$, where
$\bM_{n, (s, a)}$ denotes the potential outcome of unit $n$ for (state, action) $ = (s, a)$ (e.g. $\text{Q-learning}_n(x, a)$, $\Ex_n[x' | x, \text{do}(a)]$).
%
Assume $\bM$ has the following factorization:
%
\begin{align}
    \bM_{n, (s, a)} = \sum^R_{r = 1} u_{nr} v_{(s, a), r}
\end{align}
%
Using the SVD of $\bM$
%
\begin{align}
    \bM &= \bU \bSigma \bV^T 
    %
    \\\implies \bM \bM^T &= \bU \bV^T \bSigma^2 \bV \bU^T = \bU  \bSigma^2 \bU^T := \widetilde{\bU} \widetilde{\bU}^T,
\end{align}
%
where $\widetilde{\bU} = \bU \bSigma^{1/2}$.
%
Hence $\bM \bM^T$ functions as a (weighted) similarity matrix between the units.

%
$$
[\bM \bM^T]_{n_1, n_2} = \langle \tilde{u}_{n_1}, \tilde{u}_{n_2} \rangle
$$ 
is the (weighted) cosine similarity between the latent factors associated with units $n_1$ and $n_2$.


Assume we know $\langle \tilde{u}_{n_1}, \tilde{u}_{n_2} \rangle$ (and/or $\langle u_{n_1}, u_{n_2} \rangle$) perfectly, then does that allow us:
\begin{enumerate}
    \item Q1: learn $u_n$ for $n \in [N]$?
    \item {\bf Q2: assuming $u_1 = \sum_{j \in \Ic^{(x, a)}} \beta_j u_j$, learn $\beta$?}
\end{enumerate}
%


==> content/empirics.tex <==
\section{Empirics}

==> content/identification.tex <==
\section{A Causal Framework for Matrix Completion}\label{sec:causal_framework}
%
In this section, we develop a formal causal framework for matrix completion.
%
We state and justify our main assumptions in Section~\ref{sec:framework_main_assumptions}, define the target causal parameter of interest in  Section~\ref{sec:framework_causal_parameters}, and provide an identification proof for this parameter in Section~\ref{sec:framework_identification}.
%
We believe our framework gives a unified causal view for a variety of applications that can be posed as matrix completion problems with MNAR data, including the applications discussed in  Section~\ref{sec:motivating_applications}.

{\bf Potential outcomes framework.}
%
To begin, we use the potential outcomes framework of \cite{neyman, rubin}.
%
We associate with each row $i$ and column $j$, a r.v. $Y^{(ij)} \in \Rb$, which denotes the potential outcome associated with entry $(i, j)$, had it been revealed.
%
In the case of recommender systems, $Y^{(ij)}$ can be interpreted as the potential rating had user $i$ rated item $j$.
%
In sequential decision-making settings, $Y^{(ij)}$ can be interpreted as the potential outcome had unit $i$ undergone intervention $j$ (here we abuse notation and use $j$ to refer to both the intervention and the time period).

\subsection{Main Assumptions}\label{sec:framework_main_assumptions}
%
Recall the definitions of $\bA, \bD, \bY, \bE$ from  Section~\ref{sec:problem_setup}.

{\bf SUTVA.}
%
\begin{assumption}[SUTVA] \label{assump:sutva} 
For every $(i,j)$, 
\begin{align}
   Y_{ij} &= \begin{cases}
        &Y^{(ij)}, \text{ if } D_{ij} = 1
        \\
        & \star, \text{ otherwise.} 
    \end{cases}
\end{align}    
\end{assumption}
%
This is a standard assumption made in the causal inference literature.
%
Note that Assumption~\ref{assump:sutva} and \eqref{eq:problem_setup} together imply that 
%
$Y^{(ij)} = A_{ij} + \varepsilon_{ij},$
%
which in turn implies that $\Ex[Y^{(ij)}] = A_{ij}$ (recall, we assume $\Ex[\varepsilon_{ij}] = 0$).
%
That is, $A_{ij}$ can be interpreted as the {\em expected potential outcome} associated with entry $(i, j)$.

{\bf Latent factor model.} 
%
\begin{assumption}[Latent Factor Model]\label{assump:LFM}
For every $(i,j)$, 
\begin{align}
    A_{ij} = \Ex[Y^{(ij)}] = \langle u_{i}, v_{j} \rangle,
\end{align}
where $u_i, v_j \in \Rb^r$ are latent factors.
\end{assumption} 
%
This is a standard assumption in the matrix completion literature requiring that $\bA$ has a low-dimensional latent factor model representation, i.e., is low-rank.
%
% Such an assumption is also made in the panel data literature, and is known as a interactive fixed effects model.

{\bf Linear span inclusion.}
%
Let $\Ic_{j}$ denote the subset of rows for which column $j$ is not missing, i.e., $\Ic_{j} = \{i \in [N]: D_{ij} = 1  \}$. 
% 
\begin{assumption} [Linear span] \label{assump:linear_span} 
%
For a given $(i, j)$, for any $\Ict_{j} \subseteq \Ic_{j}$ such that $| \Ict_{j} | \ge \tilde{r}$, there exists   $\beta \in \Rb^{|\Ict_{j}|}$ such that 
%
\begin{align}
    %
	u_i = \sum_{n \in \Ict_{j}} \beta_{n} \cdot u_n ~|~ \bD. 
	%
\end{align}  
%
\end{assumption}
%
Given Assumption~\ref{assump:LFM}, we note Assumption~\ref{assump:linear_span} is rather weak.
%
Consider the matrix of row latent factors $[u_{n} : n \in \Ict_{j} \cup \{ i\}] \in \Rb^{(|\Ict_{j}|+1) \times r}$, where we recall $u_{n}$ is r-dimensional. 
%
If $r = o(\tilde{r})$, then by definition of matrix rank, Assumption~\ref{assump:linear_span} almost always holds.
%
In the worst case, it fails for at most $r - 1$ rows in the matrix $[u_{n} : n \in \Ict_{j} \cup \{ i\}]$.
%
In other words, Assumption~\ref{assump:linear_span} rules out the pathological case where row $i$'s latent factor is orthogonal to the subspace spanned by the latent factors $\{u_{n} : n \in \Ict_{j}\}$.
%
Practically, this requires that the missingness pattern $\bD$ is such that there are sufficiently many rows for which column $j$ is revealed and that the row latent factors are collectively ``diverse'' enough.


%
We emphasize that it suffices for Assumption~\ref{assump:linear_span} to hold with respect to the column latent factors rather than the row latent factors, i.e., $v_{j}$ lies in the linear span of the column latent factors for which row $i$ is revealed.
%
In such a case, one can equivalently take the transpose of the matrix and arrive back at the current formulation of Assumption~\ref{assump:linear_span}. 
% %
% In {\color{blue} Section~\ref{sec:estimator}} in particular, we discuss how to optimally create the mutually disjoint subsets $\{I_{j1}, \dots, I_{jk}\}$ from $\Ic_j$, and show two illustrative examples in {\color{blue} Figure~\ref{fig:sparsity_eg_1} and~\ref{fig:sparsity_eg_2}}.
%

% mean independence
\begin{assumption} [Conditional mean independence]\label{assump:mean_ind}
%
Let $\LFc = \{u_i, v_j \}_{i \in [N], j \in [M]}$ and $\bE = [\varepsilon_{ij}]_{i \in [N], j \in [M]}$. 
%
Let $\Ec = \{\LFc, \bD\}$.
%
Then,
%
\begin{align}
	\Ex[ \bE~|~\LFc] &= 
	\Ex[ \bE~|~\Ec] = 0.
\end{align} 
%
\end{assumption} 
%
Note that Assumption~\ref{assump:sutva} and~\ref{assump:LFM} imply that $Y^{(ij)} = \langle u_i, v_j \rangle + \varepsilon_{ij}$.
%
In turn, Assumption~\ref{assump:mean_ind} implies that $\Ex[Y^{(ij)}~|~\LFc] = \Ex[Y^{(ij)}~|~\Ec]$.
%
That is, conditional on the latent factors, the potential outcomes $Y^{(ij)}$ are mean independent of the ``interventions'', $\bD$.
%
Analogous to the selection on observables assumption that is standard in causal inference, this can be interpreted as a  ``selection on latent factors'' assumption.
%
We stress that the latent factors, $\LFc$, and the intervention assignments, $\bD$, can be mutually dependent, and we make no assumptions about the structure of their dependencies.

%
% The crucial conditional independence required is that $\bD \independent \bE ~|~ \LFc$.
% %
% In Figure~\ref{fig:causal_DAG}, we give one example of a directed acyclic graph (DAG) that is concordant with Assumption~\ref{assump:mean_ind}.
% %
%
% \begin{figure}
% \centering
% \includegraphics[width=0.30\textwidth]{images/DAG.png} 
% \caption{DAG representation}
% \label{fig:causal_DAG}
% \end{figure}
 
\subsection{Target Causal Parameter}\label{sec:framework_causal_parameters}
%
We are now equipped to define our main causal parameter of interest.
%
It is the expected potential outcome for entry $(i, j)$ of the matrix, conditioned on the latent factors, $u_i, v_j$ (i.e., row $i$ and column $j$'s latent factors).
%
That is,
\begin{align}\label{eq:cauasal_param_entry_wise}
    \theta^{(ij)} \coloneqq \Ex[Y^{(ij)} ~|~ u_i, v_j]
\end{align}
%
For example in recommender systems, this would refer to the potential rating associated with user-item $(i, j)$, conditioned on the user specific and item specific latent factor.

%
In Section~\ref{sec:other_causal_params}, we discuss the identification and estimation of other causal parameters that might of interest in different applications of matrix completion.
%
We also discuss the trade-offs associated with estimating these various parameters in terms of the requirements placed on $\bD$.

% IDENTIFICATION 
\subsection{Identification}\label{sec:framework_identification} 
%
\begin{theorem}\label{thm:identification}
For a given $(i, j)$, let Assumptions \ref{assump:sutva} to \ref{assump:mean_ind} hold. 
%
Further, for a given subset $\Ict_{j} \subseteq \Ic_{j}$, suppose $\beta$ is known. 
%
Then, 
\begin{align}
	\theta^{(ij)} &= \sum_{n \in \Ict_{j}} \beta_{n} \Ex\left[ Y_{n j} ~|~ \Ec\right].
\end{align} 
\end{theorem} 

\begin{proof}
In what follows, the descriptors above the equalities represent the assumption used, e.g., $A1$ represents Assumption 1: 
\begin{align} 
    %
	\theta^{(ij)} &= \Ex[Y^{(ij)}~|~u_i, v_j]
	%
	\\ &\stackrel{A2}= \Ex[\langle u_i, v_j \rangle + \varepsilon_{ij} ~|~ u_i, v_j] 
	%
	\\ &\stackrel{A4}= \langle u_i, v_j \rangle  ~|~ \{u_i, v_j\} 
	%
	\\ &
	= \langle u_i, v_j \rangle  ~|~\Ec 
	%
	\\ &\stackrel{A3}= \langle \sum_{n \in \Ict_{j}} \beta_{n} u_n,  v_j \rangle  ~|~\Ec
	%
	\\ &\stackrel{A4}=  \sum_{n \in \Ict_{j}} \beta_{n} \Ex\left[ \left( \langle u_n, v_j \rangle + \varepsilon_{n j} \right)~|~\Ec\right] 
	%
	\\ &\stackrel{A2}= \sum_{n \in \Ict_{j}} \beta_{n} \Ex\left[ Y^{(n j)} ~|~\Ec\right]
	%
	\\ &\stackrel{A1}= \sum_{n \in \Ict_{j}} \beta_{n} \Ex\left[ Y_{n j} ~|~\Ec\right]. 
	%
\end{align} 
\end{proof} 
% %
% As an immediate consequence of \eqref{eq:cauasal_param_row_wise}, Theorem~\ref{thm:identification} serves as an identification argument for $\bar{\theta}^{(i)}$ as well.
%
Theorem~\ref{thm:identification} states that given knowledge of $\beta$, it is possible to write $\theta^{(ij)}$ as a linear combination of observable quantities; this is true since for $n \in \Ict_{j}$, $Y_{n j} \neq \star$ (i.e., is not missing).
%
Next, in Section~\ref{sec:estimator} we provide a simple procedure to estimate $\theta^{(ij)}$.
%





==> content/motivating_applications.tex <==
\section{Example Applications} \label{sec:applications}

%{\color{red}
%1. panel data pattern; 
%2. checker-box; 
%3. special case of MAR --> implications for MCAR
%}

\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.29\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/staircase.jpg}
		\caption{\smaller Recommender systems.} 
		\label{fig:staircase}
	\end{subfigure} 
	\qquad \qquad 
	\begin{subfigure}[b]{0.43\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/sequential.jpg}
		\caption{\smaller Sequential decision-making.} 
		\label{fig:panel} 
	\end{subfigure} 
	\caption{\smaller In both \ref{fig:staircase} and \ref{fig:panel}, observed entries are shown in yellow while unobserved entries are shown in white. Further, in \ref{fig:panel}, the columns are indexed by (time, policy) tuples; here, $t_\ell$ and $p_\ell$ denote the $\ell$-th time period and policy, respectively. 
	}
	\label{fig:obs_patterns} 
\end{figure}

%
In this section, we highlight a few important real-world applications that can be posed as matrix completion with MNAR data. 
%
We describe the missingness patterns that are typical of these applications and argue why the current suite of matrix completion methods in the literature are ill-equipped to handle these settings, at least in terms of their theoretical analyses.
%
Ultimately, these examples reinforce the need for a new causal framework for matrix completion with MNAR data, such as the one we present in Section~\ref{sec:causal_framework}.
%

{\bf Recommender systems.} 
%
As stated earlier, one of the key motivating applications for matrix completion is recommender systems.
% 
In these settings, it is well noted that observations are often subject to selection-biases as users naturally consume items that they enjoy and avoid items that they dislike. 
%
In an extreme version of this scenario, users will behave entirely binary in this respect, which would induce a sparsity structure as shown in Figure~\ref{fig:staircase}. 
%
Within the context of movie recommender systems, a narrative for this missingness pattern is one in which users, in general, only watch films that belong to genre(s) that they like and nothing else. 
%
However, due to their influence on pop culture, there is a small subset of core, iconic films (e.g., {\em Titanic} or {\em Star Wars}) that all users have watched; pictorially, this is represented by the fully observed submatrix at the bottom of Figure~\ref{fig:staircase}. 
%
Another example for the dense submatrix is one in which platforms ask new users to indicate a subset of films that they enjoy. 
%
Indeed, this is a common practice for online platforms such as {\em Hulu} to quickly learn a new user's preferences in order to provide a ``warm-start'' to their recommendation engine. 

Though the example in Figure~\ref{fig:staircase} is obviously an extreme caricature, it highlights some of the critical limitations of the current suite of matrix completion techniques. 
%
Specifically, the standard literature assumptions of (i) $D_{ij} \independent D_{ab}$ for all $(i,j) \neq (a,b)$ and (ii) $p_{ij} > 0$ are clearly violated since 
(i) conditional on knowing that user $i$ has rated a movie from a particular genre, it deterministically reveals the values of the remaining entries in the $i$-th row of $\bD$,
and (ii) $\min p_{ij} = 0$ by construction. 
%
In contrast, the causal framework we present in Section~\ref{sec:causal_framework} allows for both conditions to hold.  
%
As such, our framework allows for the extreme caricature, or aspects thereof, to exist within the observed dataset, and our proposed \SNN~algorithm can provably recover the underlying expected potential outcomes matrix, provided $\bY \independent \bD ~|~ \{\bU, \bV\}$. 
%
{\color{red} low-dimensional} 


{\bf Panel data.}

{\bf Sequential decision-making.} 
Compared to recommender systems, a possibly less intuitive application of matrix completion with MNAR data is sequential decision-making.
%
Here, data is collected across units (e.g., individuals, customer types) over time in a sequential manner, where each unit is likely to be observed under a single or small set of interventions out of many at any time period. 
%
%As described briefly earlier, consider a scenario where we collect data of different units (e.g. individuals, customer types, geographic locations) in a sequential manner, and at each time period we observe each unit under some intervention.
%
Many sequential decision-making problems can be phrased this way, including
%
(i) panel data settings in econometrics;
%
(ii) reinforcement learning and its variants (e.g., online learning, contextual bandits); 
%
(iii) sequential A/B testing. 
%
In (ii), an intervention denotes both the action picked and the observed state for that given time period; 
%
meanwhile in (iii), platforms run experiments on different customer types in a sequential and/or adaptive manner over time.
%
The induced matrix in these settings has rows index units and columns index time-intervention pairs; for an illustration, see Figure~\ref{fig:panel}. 
%
An important goal in such scenarios is to impute this induced matrix, i.e., estimate the counterfactual outcome of what would have happened to each unit, at each time period, under all interventions of interest.

%{\bf Limitations of current methods.}
%%
%Like we do in the recommender system example, we next list why the current literature on matrix completion with MNAR data cannot handle such settings.
%%
As with the recommender system example, the current literature on matrix completion with MNAR data cannot handle these settings due to the following reasons: 
% 
(i) The entries of $\bD$ are not independent; if a unit receives a particular intervention at a time period, then we deterministically know that it cannot have received any other intervention at that same time period. {\color{red} how about ecommerce a/b testing example where same customer group received all discounts during same 8 day span? change to individual} 
%
(ii) $\min p_{ij} = 0$; this will be true for example if a unit deterministically goes through a particular intervention at some time period (e.g., all units do not undergo any intervention in the first time period, i.e., remain under ``control'').
%
{\color{red} low-dimensional} 
%
%(iii) $\bD \notindep \bA$; in many sequential decision-making settings, one only has access to {\em offline, observational} data; hence, outside purely experimental settings, there is likely hidden correlation between which interventions a unit goes through at a time period and their potential outcome (e.g. discount policies might by given to users that are likely to spend more/less on a platform).
%%
%(iv) $\Ex[\bD]$ is not low-rank; if there are a large number of units and possible interventions, just like Figure~\ref{fig:non_low_rank}, it is easy to construct scenarios where $\Ex[\bD]$ is not low-rank.
%%
%





==> content/other_parameters.tex <==
\section{Other Causal Parameters of Interest}\label{sec:other_causal_params}
%
Apart from $\theta^{(ij)}$, there can be many causal parameters of interest in matrix completion, depending on the application.
%
We focus on $\theta^{(ij)}$ as it is arguably the most challenging causal parameter to estimate, i.e., the potential outcome associated with each row $i$ and column $j$.
%
However, the trade-off is that other causal parameters of interest require us making weaker assumptions about $\bD$, the observed missingness pattern.
%
Below, we explore this trade-off through the following causal parameter, which is the expected potential outcome associated with a given subset of entries for a given row $i$.
%
That is,
\begin{align}\label{eq:cauasal_param_row_wise}
    \bar{\theta}^{(i)} \coloneqq \frac{1}{| U|} \sum_{j \in U_i} \Ex[Y^{(ij)} ~|~ u_i, v_j] =  \frac{1}{| U_i|} \sum_{j \in U} \theta^{(ij)},
\end{align}
where $U \subset [M]$.
%
The particular subset of $U$ that this is average is taken over is application dependent.
%
For example in movie recommender systems, $U$ could be taken to be one particular genre of movies---this might be of interest to a platform to make movie recommendation decisions.
%
$U$ could also be taken to be $\{j: D_{ij} \neq 1\}$, i.e., the subset of all movies that user $i$ has not rated---this might for example be of interest to a platform in deciding which users to give a discount policy to.
%
In panel data settings, $U$ could refer to some subset of the observed time periods.

%
\subsection{Variant of SI-MC Estimator for $\bar{\theta}^{(i)}$}\label{sec:other_causal_param_algorithm}

%
{\bf Largest square sub-matrix induced from $\Ic_{j}$.}
%
To estimate $\bar{\theta}^{(i)}$, the key difference is that we do not require creating $K$ disjoint subsets from $\Ic_j$ for each $j \in U$, as long as $U$ is growing (recall $U \subset [M]$).
%
In particular, for each subset $\tilde{\Ic}_j \subset \Ic_j$, define $\tilde{\Omega}_i$ where
$$
\tilde{\Omega}_i = \{m \in [M]: D_{i, m} = 1 \text{ and } D_{n, m}=1 \text{ for all } n \in \tilde{\Ic}_j \}.
$$
%
To estimate $\bar{\theta}^{(i)}$ it suffices to find the single subset of $\Ic_j$, which we denote as $\Ic^*_{ij}$, such that
$$
\Ic^*_{ij} \coloneqq \max_{\tilde{\Ic}_j \subset \Ic_j} \min\{ |\tilde{\Ic}_j|, |\tilde{\Omega}_i| \}.
$$
%
Define $\Omega^*_{ij}$ with respect to $\Ic^*_{ij}$, analogous to how $\tilde{\Omega}_i$ is defined with respect to $\tilde{\Ic}_j$.
%
As an illustration of the difference between the construction of $\Ic^*_{ij}$ and $\{\Ic_{j1}, \dots, \Ic_{jk}\}$, in Figure~\ref{fig:sparsity_eg_1}, we can take $\Ic^*_{ij} = \bigcup^K_{k = 1} \Ic_{jk}$ (and $\Omega^*_{ij} = \Omega_{i, 1}$).

%
Let 
$$Y_{\Omega^*_{ij}} = [Y_{im}:  m \in \Omega^*_{ij}] \in \Rb^{|\Omega^*_{ij}|},$$
%
$$Y_{\Ic^*_{ij}} = [Y_{n j}:  n \in \Ic^*_{ij}] \in \Rb^{|\Ic^*_{ij}|},$$
%
$$\bY_{\Ic^*_{ij}, \Omega^*_{ij}} = [Y_{n m}: n \in \Ic^*_{ij}, m \in \Omega^*_{ij}] \in \Rb^{|\Ic^*_{ij}| \times |\Omega^*_{ij}|  }.$$
%
Lastly, denote the singular value decomposition (SVD) of $\bY_{\Ic^*_{ij}, \Omega^*_{ij}}$ as: 
\begin{align}
    \bY_{\Ic^*_{ij}, \Omega^*_{ij}} &= \sum_{\ell=1}^{S_{ij}} \hlambda^{ij}_{\ell} \hvarphi^{ij}_{\ell} \otimes \hv^{ij}_{\ell}. 
\end{align}
where $S_{ij} = \min\{|\Ic^*_{ij}|, |\Omega^*_{ij}| \}$. 


{\bf Estimating $\bar{\theta}^{(i)}$.} 
%
Below, we state our estimation procedure. 
%
There is one hyper-parameter $q_{ij} \in [S_{ij}]$, which refers to the number of principal components we retain of $\bY_{\Ic^*_{ij}, \Omega^*_{ij}}$.
%
\begin{enumerate}
    % PCR
    \item Estimating $\beta_i$: 
    \begin{align} \label{eq:pcr_regular}
        \hbeta_i = \Big( \sum_{\ell=1}^q (1/ \hlambda^{ij}_{\ell}) \hv^{ij}_{\ell} \otimes \hvarphi^{ij}_{\ell} \Big) Y_{\Omega^*_{ij}}. 
    \end{align}
    
    % Counterfactual
    \item Estimating $\bar{\theta}^{(i)}$:
    \begin{align} \label{eq:si_regular} 
        \widehat{\bar{\theta}^{(i)}} = \frac{1}{|U|} \sum_{j \in U} \htheta^{(ij)},
    \end{align}
    where $\htheta^{(ij)} = \langle \hbeta_i,  Y_{\Ic^*_{ij}}\rangle$
\end{enumerate}
%
{\bf Interpretation.}
%
In comparison, to estimate $\bar{\theta}^{(i)}$, which can be expressed as the average of many entries of the matrix (assuming that the set $U$ is sufficiently large), we do not need to create these $K$ separate estimators.
%
This is because taking the average over the the columns in $U$ implicitly performs this ``bootstrapping'' step.
%
More generally, the trade-off is as follows.
%
$\theta^{(ij)}$ is clearly a more challenging causal parameter to estimate, as $\bar{\theta}^{(i)}$ is simply the average of  $\theta^{(ij)}$ over $j \in U$. 
%
However, to estimate $\theta^{(ij)}$, we make a more stringent requirement of the missingness pattern $\bD$.
%
As we establish in Section~\ref{sec:theoretical_results}, to estimate $\theta^{(ij)}$ we require $\bD$ to be such that there exists $K$ disjoint subsets such that $\min_{k \in [K]} \{|\Ic_{jk}|, |\Omega_{ik}|\}$ is sufficiently large, and that $K$ is growing as well.
%
In comparison, to estimate $\bar{\theta}^{(i)}$, we simply require finding one sufficiently large sub-matrix (i.e., $\bY_{\Ic^*_{ij}, \Omega^*_{ij}}$) to estimate $\htheta^{(ij)}$ for each $j \in U$. 


{\color{red}
%
\subsection{Theoretical results for $\bar{\theta}^{(i)}$}\label{sec:other_causal_param_theory}
}

==> content/simulations.tex <==
\section{Simulations}
